LaGeM: A Large Geometry Model for 3D Representation Learning and Diffusion

This paper introduces a novel hierarchical autoencoder that maps 3D models into a highly compressed latent space. The hierarchical autoencoder is specifically designed to tackle the challenges arising from large-scale datasets and generative modeling using diffusion. Different from previous approaches that only work on a regular image or volume grid, our hierarchical autoencoder operates on unordered sets of vectors. Each level of the autoencoder controls different geometric levels of detail. We show that the model can be used to represent a wide range of 3D models while faithfully representing high-resolution geometry details. The training of the new architecture takes 0.70x time and 0.58x memory compared to the baseline. We also explore how the new representation can be used for generative modeling. Specifically, we propose a cascaded diffusion framework where each stage is conditioned on the previous stage. Our design extends existing cascaded designs for image and volume grids to vector sets.

==> data/geo_form.tex <==
\def\arraystretch{1.15}\tabcolsep=0.32em
\begin{tabular}{ccc}
\toprule
& Geometric Quality & Network Arch \\ \midrule
Volume & Low & Conv \\
\rowcolor{mytbcol!30}Sparse Volume & High & SparseConv \\
Irregular Grid & High & Transformer \\
\rowcolor{mytbcol!30}VecSet & High & Transformer \\ \bottomrule
\end{tabular}

==> data/geo_learn.tex <==
\def\arraystretch{1.15}\tabcolsep=0.32em
\begin{tabular}{ccc}
\toprule
& To Latent & Training \\ \midrule
\rowcolor{mytbcol!30}Per-Object Opt & Slow & No \\ 
AutoDecoder & Slow & Yes \\
\rowcolor{mytbcol!30}AutoEncoder & Fast & Yes \\
\bottomrule
\end{tabular}
